Towards Automating Precision Studies of Clone Detectors

Current research in clone detection suffers from poor ecosystems for evaluating precision of clone detection tools. Corpora of labeled clones are scarce and incomplete, making evaluation labor intensive and idiosyncratic, and limiting inter tool comparison. Precision-assessment tools are simply lacking. We present a semi-automated approach to facilitate precision studies of clone detection tools. The approach merges automatic mechanisms of clone classification with manual validation of clone pairs. We demonstrate that the proposed automatic approach has a very high precision and it significantly reduces the number of clone pairs that need human validation during precision experiments. Moreover, we aggregate the individual effort of multiple teams into a single evolving dataset of labeled clone pairs, creating an important asset for software clone research.

==> approach.tex <==
\section{Clone Validation vs. Clone Detection}
\label{sect:approach}

There is a subtle but important difference between a clone pair
validator and a clone detector. A clone detector's aim is to find
(detect) the clone pairs in a dataset presented to it. There is a
component which works on the retrieval of information from the
dataset. For this reason, a good clone detector needs to have good
recall as well as good precision. A good clone detector should also be
able to scale to large datasets, otherwise it is of little use for
practical purposes. 

In contrast, a clone pair {\em validator} only needs to decide whether
a given pair is a clone or not. The input to a clone validator is not
a potentially large dataset of code, but a dataset of
candidate clone pairs that may or may not be clones.\footnote{A
  candidate pair consists of two piece of code reported as clone pair by a
clone detection tool. Our approach validates these pairs, and only
when they are resolved as true positives they are called clone pairs.} Typically, researchers
estimate the precision of clone detectors by manually analyzing a
statistically random sample of candidate pairs from the output of the
clone detector. Hence, a clone validator designed to facilitate this
validation process also needs to evaluate only a random and
statistically significant sample of candidate pairs. As a result, there is
no need to address the problem of scalability.


An automatic approach to validating candidate pairs must be able to
resolve the pairs presented to it with perfect precision. With this
in mind, we designed the automatic mechanism of our approach to
have a very high precision and compromised on its recall, simply
because recall is not important for clone validators.

We note that clone detection tools operate at various granularities
like statements, block of code, methods, files, et cetera. Also, clone
detection can be carried out for software written in various languages
like C, C++, and Python among others. In this work, we narrow down
our focus to facilitate precision studies for method level clone
detectors which find clones in software systems written in Java.
% We made this decision because we already have experience with
% designing and creating method level clone detection tools. Moreover,
% many fast and scalable state of the art clone detection tools are
% capable of method level clone detection tools and they also find
% clones on software written in Java. There is a popular dataset
% called BigCloneBench~\cite{bcb}, a real world benchmark of manually
% validated method level clones in the
% IJaDataset-2.0~\cite{ijadataset} (25,000 Java systems).

 


==> architecture.tex <==
\subsection{Architecture of InspectorClone}
\label{sect:architecture}

The architecture of \IC\ can be seen in Figure \ref{fig:architecture}. It is composed by a Django\footnote{Django is a Python web framework: https://www.djangoproject.com} application that is connected to a set of databases and provides functionality.

There are two databases in the back-end of \IC. One, BCB, includes the code clone information of the BCB dataset as described earlier. It is used as a starting point for adding new knowledge regarding clones and does not have any special utility beyond this. The second database is used to store contextual information like registrations, users, and so on; and newly added information about true or false clone pairs, and their clone types if applicable. This second database is the main point of information storage in \IC. Future improvements of BCB can simply replace the older version of the BCB database in \IC.

% A corpus of source code is also provided through IC. This dataset is the same as the one that was used to create BCB and is provided to allow different users with different tools to perform an analysis on the same information. It is the 'shared input' across multiple analysis.

\begin{figure}
  \centering
    \includegraphics[scale=0.4]{figures/pf-architecture.png}
  \caption{Architecture of IC.}
  \label{fig:architecture}
\end{figure}

Just like for BCE, the information uploaded to \IC, namely the result
of running a certain clone detection tool, must follow a specific
format, in the form of a Comma Separated Values (CSV) file with the
following columns: \texttt{folder\_name\_1}, \texttt{file\_name\_1},
\texttt{start\_line\_1}, \texttt{end\_line\_1},
\texttt{folder\_name\_2}, \texttt{file\_name\_2},
\texttt{start\_line\_2}, \texttt{end\_line\_2}. Note that the first
four columns repeat themselves as the second four columns, to describe
both sides of a (clone) pair.

Through the web application, \IC\ provides users and judges with an
interface to carry out precision studies of their clone detector
tools. The data, at any given point, is available to any user who wants
it, together with the source code itself, in order to facilitate use
in isolation (though not encouraged) or for derivative work.




==> improving-pf.tex <==
\section{Knowledge Improvements by InspectorClone}
\label{sect:improve}

In facilitating precision studies, InspectorClone also improves the
existing clone labeling contained in BCB in two ways: \IC\ contains an
automatic mechanism to detect Type I clone pairs and it contains a
large dataset of Type II clone pairs manually validated by us. The
goal behind these additions is to minimize as much as possible the
number of clone pairs shown to human judges. These two optimizations
are described in this section.

\subsection{Automatic Type I Resolution} \label{subsect:auto-type-2}

Recent research suggests that Type I clones are significantly abundant
in and across software systems~\cite{Lopes:2017:DMC:3152284.3133908},
at least at file level. while we are concerned here with method level,
methods are elements of files and therefore, the results can be
extrapolated to method-level. What is relevant is that the number of Type I clones is
overwhelming. This means that if one wants to do a precision study of
their tool, there will be a significant large number of Type I clone pairs
requiring manual validation.
 %Figure \ref{fig:java-clone-pie}\footnote{Image provided with the authorization from the authors.} 

%Recent research suggests that Type I clones are significantly abundant in and across software systems~\cite{Lopes:2017:DMC:3152284.3133908}. Take for example, Figure \ref{fig:java-clone-pie}\footnote{Image provided with the authorization from the authors.} from a recently published large-scale clone analysis work. What is labeled as 'Duplicated', actually refers to Type I pairs. (in the same figure, 'Cloned' means number of files that are clones with a degree of variation, 'Unique' refers to elements without clones). 

%\begin{figure}
%  \centering
%    \includegraphics[scale=0.15]{figures/java-pie-chart.png}
%  \caption{Distribution of clone types for all the Java projects in GitHub, as seen in D\'ej\`aVu \cite{Lopes:2017:DMC:3152284.3133908}. Information for file clones, not method clones.}
%  \label{fig:java-clone-pie}
%\end{figure}

Thankfully, Type I clones are easy to detect automatically. As
described in Section \ref{subsect:clone_types}, the definition of Type
I clones says two pairs are Type I clones if they are exact replicas
when neglecting source code comments and layout\footnote{The syntax of
  Java is not dependent on layout, so we can ease the definition of
  Type I clones. For layout-dependent syntaxes like the ones found in
  Python or Haskell, this approach would require a more careful
  deliberation}. This makes the validation of Type I clones similar to
a simple string comparison after removing certain
elements. Following this logic, in the background of \IC, we have
implemented an automatic mechanism for Type I detection. Starting with
an unseen clone pair candidate, this mechanism performs the following
tasks:

\begin{enumerate}

\item{For each side of a clone pair, remove all the source code comments.}

\item{For each side of a clone pair, normalize the layout by removing white spaces and newlines.}

\item{Hash both strings using the SHA-256 hashing algorithm.\footnote{The url~\url{https://docs.python.org/2/library/hashlib.html\#module-hashlib} points both to the library used and to the definitions of the algorithm.}}

\item{Compare both hashes, if they are the same, automatically flag the pair as a true clone relation.\footnote{Since these algorithms have a cryptography background, we deemed the likelihood of hash collisions for the purposes of clone detection statistically irrelevant.}}

\end{enumerate}

The usage of hash instead of string comparison has to do with backend optimizations: this way we can save the hashes of known clone elements, avoiding the negative performance effects of constant large-scale parsing, handling and hashing.

This leverages a large amount of work from the users since a large number of clones are Type Is, and these are automatically resolved by the system. If \IC\ find that a pair is not a Type I clone, and the pair is not marked as a clone in either BCB or \IC, then it forwards the pair through the standard mechanism of manual judging.

\subsection{Addition of Type II clones} \label{subsect:type2-addition}

The definition of Type II clones implies that they are more complex
than Type I clones: we can not perform simple string refactoring and
hash comparisons. However these are easier to detect than Type III and
Type IV clones (Type IV being clearly the hardest). This relative
simplicity of Type II clones has resulted in the availability of clone
detection tools that are capable to detect them; in fact, there are
tools that have been shown to have almost or near 100\% recall in this
category ~\cite{Svajlenko:2015:ECD:2881297.2881379,
  svajlenko2017fast}. The availability of techniques to detect Type II
clones opens an opportunity: we can run tools on the entire dataset,
intersect their results, sample the intersection and manually validate
it. That is what we did.

We used two well-known, state of the art clone detection tools: NiCad
and CloneWorks. NiCad ~\cite{roy2008nicad} is a near-miss clone
detector that works by extracting the smallest pieces of code that can be
considered as clones. Then, a pretty printing is applied to code
pieces; this includes breaking different parts of a statement to
multiple lines, normalization of code to ignore the editing
differences, and filtering out uninteresting statements from potential
clones. Next, potential clones are compared using Longest Common
Subsequence algorithm, and clone pairs are identified and reported.

CloneWorks ~\cite{svajlenko2017fast} is a hybrid tool based on token-
and index-based approaches. It has two components: input builder, which
extracts the code fragments, and a clone detector. The clone detection
component creates a global token frequency map of tokens, and uses it
to create an inverted partial-index of code blocks using the sub-block
filtering. It uses a modified Jaccard similarity metric in which
similarity is measured as the minimum overlap ratio between tokens of
two blocks.

We ran these tools on the entire dataset to get only Type II clones
from them. CloneWorks has mechanisms for reporting only Type II
clones; for NiCad, we ran it once to get Type I clones, and once again
to get Type I and Type II clones, then we extracted Type II clones by
removing the Type I's. The results obtained after these efforts are
presented in Table \ref{table:clone-tools-type2}.

\begin{table}[]
\centering
\caption{Type II clones found by NiCad and CloneWorks, individually and together.}
\label{table:clone-tools-type2}
\begin{tabular}{|l|r|}
\hline
\multicolumn{1}{|c|}{} & \# Type II Clones \\ \hline \hline
NiCad                                   & 336,441           \\ \hline
CloneWorks                              & 696,428           \\ \hline
Intersection                            & 159,691           \\ \hline
Intersection \textgreater 50 tokens     & 73,885            \\ \hline
\end{tabular}
\end{table}

There are 159,691 clone pairs that both tools have detected and from
these, 73,885 contain methods with 50 or more tokens. From these
73,885 pairs, we sampled 1,851 which is a statistically representative
sample size with a confidence level of 99\%, and a margin of error of
$\pm$ 3\%. Four judges (four authors from this work) went through this
sample to ensure all the elements were true Type II clones, after
which the 73,885 clones were added to \IC.

\subsection{Known Clones}

On Table~\ref{table:known-clones}, we can see all the information
added. Combining with BCB, we now know 78,462 Type II
clones. \IC\ only inherits a subset of Type III clones from BCB.

In the recall summary of BCE, it classifies Type III clones into
further subcategories based upon the syntactic similarity of methods
in clone pairs. They define these subcategories as, quoting original
work: ``Very-Strongly Type-3 clones (VST3) as those with a similarity
in range 90\% (inclusive) to 100\% (exclusive), Strongly Type-3 (ST3):
70-90\%, Moderately Type3 (MT3): 50-70\%, and Weakly Type-3/Type-4
(WT3/4): 0\%-50\%''~\cite{Svajlenko:2014:TBD:2705615.2706134}.

However, BCB only categorizes clone pairs into Type I, Type II, and
Type III. The Type IV clones that BCE reports are not manually validated
by humans; they are labeled based on the similarity rate from Type III
clones and treated the same as Weakly Type III clones.

\IC\ inherits all clones (19,187) from the first two subcategories
which are VST3 and ST3 (more than 70\% similar). As the syntactic
similarities between two methods decreases, the methods become harder
to judge, and we want the users of \IC\ to make the final judgement
about such pairs.


\begin{table}[]
\centering
\caption{Total number of clones known by \IC.}
\label{table:known-clones}
\begin{tabular}{|c|c|c|c|}
\hline
                                                       & Type I & Type II                                                           & Type III \\ \hline \hline
\begin{tabular}[c]{@{}c@{}}Known\\ Clones\end{tabular} & all    & \begin{tabular}[c]{@{}c@{}}78,462\\ (4,577 from BCB)\end{tabular} &  \begin{tabular}[c]{@{}c@{}}19,187\\ (all from BCB)\end{tabular} \\ \hline
\end{tabular}
\end{table}


==> pf.tex <==
\section{InspectorClone: Use Cases and Design} \label{sect:using}

The current method for estimating the precision of a code clone
detection tool is to manually validate a statistically significant
random sample of the clone pairs reported by the
tool~\cite{sajnani2016sourcerercc}. This is a manual effort, where a
user needs to create a random sample, and then this random sample
needs to be validated manually by a number of judges. Finally, the
judgments are aggregated, mostly using voting. InspectorClone
semi-automates this entire process. Through a web application, users
can submit the results of clone detection tools and obtain an estimate
of precision. \IC\ relies on community support to increase the
existing body of knowledge about clones on its dataset.


\begin{figure}
  \centering
    \includegraphics[scale=0.4]{figures/pf.png}
  \caption{Using InspectorClone.}
  \label{fig:using-pf}
\end{figure}

The workflow of \IC\ can be seen in Figure
\ref{fig:using-pf}. \IC\ does not run the clone detection tools
themselves. Instead, the user is responsible for downloading the
dataset of source code from \IC, run the tool on this source code
corpus, and upload its results to \IC\ following a specific
format, which is the same as the one expected by
BCE. From this moment, \IC\ will sample the results (a statistically
significant sample) and match them against the existing clone
knowledge. Sampling is done because it is a common practice in
estimating the precision of clone detectors, and also because for the
part of evaluation that demands human effort, it is not feasible to do
the experiment on the complete output of a clone detector.

\subsection{Usage Scenarios}
In the best case scenario, when all clone pairs in the sample have
already been flagged as either true or false positives, then
\IC\ simply registers the experiment and provides the user with the
tool's precision report, without further human intervention. Consider
the following scenario:

\textit{John creates Sherlocklone, a tool that detects clones. Sherlocklone has reached now a state deemed mature and John wants to validate the tool in an environment the tool has never seen.
	% and he needs to compare the tool with the solution from other research teams that are also known to perform well (looking at you, CloneCatcher). 
The solution is to go to the \IC\ website, download the dataset, run Sherlocklone on the dataset, and submit the clone results to \IC. Now, \IC\ tells John the estimated precision of his tool}.
%  in an unseen space., and can look at other experiments with other tools and compare different results.} 
%~\com{\IC\ does not have the functionality to let a user compare it's tool with the other tools. Let's not say that we offer this functionality. If a user wants to compare the precision of his tool with some other tool, he needs to setup two experiments. Each experiment for each tool. Just like how we compared precision of Nicad, CW and SCC}

In this idealized usage of \IC, \IC\ provides a central body of
knowledge which can be used to expedite precision studies by giving an
imediate precision estimate. Note that in the scenario above, John was
lucky, because all the clone pair candidates that were necessary to
validate Sherlocklone had previously been flagged (as clones or not
clones). However, this scenario is unlikely to happen, as chances are
a subset of the clone pairs reported by the tool have not been labeled
before. \IC\ is designed precisely to deal with these other situations, and
it allows John to ask for help in validating the clone pairs that are
not labeled in the database.

% \subsection{Scenario II}
% \IC\ contains a system of validation of the sampled clone pairs based on groups of judges. The owner of a certain experiment can choose any number of judges in order to manually validate the clone pairs. This round of validation goes until all the information is known, after which \IC\ provides the results.

Consider the following more likely scenario:

\textit{\IC\ told John that it could not estimate the precision of
  Sherlocklone completely on its own. Reason: some of the clone pair
  candidates the tool is reporting were never seen
  before. \IC\ provides a solution: it shows John a window where he
  can appoint registered users to help him validate the pairs not
  flagged in database. John asks his three postdocs, Erica, Peter and
  Andrew, to register on \IC\ and assist him with the precision
  experiment. After John invites them as judges to the experiment,
  Erica goes to \IC\ and logs in, and in her home page, she sees that
  she has an experiment to complete. Clicking on the experiment, she
  is presented with a window, in her browser, split in two, each side
  representing each side of a clone pair candidate. Erica has to
  decide if these are indeed clones, or not, what is their clone type
  (optional), and leave any comment she wants. When all the pairs have
  been validated by Erica, Peter, and Andrew, \IC\ aggregates their
  decisions by taking the majority vote, creates a precision report
  for Sherlocklone, and merges the knowledge originated in this
  experiment with its previously known knowledge. The next time John
  logs in, his precision study will be reported as complete, and an
  estimate of precision will be shown to him.}

This scenario represents the typical interactions with \IC. It is
expected that, as more tools are analyzed, and more teams make the
effort to manually look at unseen clone candidates, less effort will
be required, as more information is known about clone presence in the
dataset. To some extent, this process may never finish, as
advances and sophistication in clone detection techniques, and their
implementations in clone detection tools will likely find clones in
areas that were previously blurry. Furthermore, clone detection tools
will always inevitably produce some false positives, and given the
large space of possible pairs in the dataset (being clones or not),
some validation might always be required to understand unexpected and
erroneous behaviors. The frequent use of \IC\ by many researchers in the community
will help build an increasingly better labeled dataset.

This last point of aggregating multiple efforts is really at the
center of \IC. Validation is hard and error-prone. A group of humans
is the most trustful source of understanding and labeling, and
\IC\ aggregates the many individual team efforts and returns it back
to the community, both as a clone detection tool validation and as a
dataset representing a clones body of knowledge.

\subsection{\IC\ Interface}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=0.3]{figures/tool_register_screen.png}
        \includegraphics[scale=0.3]{figures/experiment_register_screen.png}
    \end{subfigure}
    
	\vspace{10px}

    %\begin{subfigure}[b]{\textwidth}
   %     \includegraphics[scale=0.17]{figures/experiment_register_screen.png}
    %\end{subfigure}

	%\vspace{10px}

    \begin{subfigure}[b]{\textwidth}
        \includegraphics[scale=0.17]{figures/judge_invite_screen.png}
    \end{subfigure}
    \caption{InspectorClone interfaces to: register a new tool (top-left), register a new experiment (top-right), and invite judges to validate clone candidates (bottom).}
	\label{fig:registration_screens}
\end{figure}
\begin{figure*}[t]
	\centering
	\includegraphics[scale=0.35]{figures/evaluate_pairs_screen.png}
	\caption{Validation of clone candidates on InspectorClone.}
	\label{fig:evaluate_pairs_screen}
\end{figure*}

Because the web interface of \IC\ is such a relevant part of the tool,
it is worth looking at parts of it in some detail. This section is
presented in the sequence on which they appear to users.

Figure \ref{fig:registration_screens} shows the options to add a new
tool, add a new experiment, and invite judges to an experiment. The
page to add a new tool (Figure \ref{fig:registration_screens},
top-left) is a simple web interface with 3 input elements, one for the
tool name, another for the tool version and a third one to add a
description of the tool. The page to add a new experiment (Figure
\ref{fig:registration_screens}, top-right) allows specifying an
experiment's name, and provides a drop down list to select a tool from
among the tools that has been previously registered (mandatory) by
this user. It also provides another mandatory input element to submit
the results of running the tool (remember, \IC\ requires the user to
download a dataset and run his/her tool on it, and upload the results in a
proper format). Results are then sampled and the experiment
starts. Finally, the same user who created the experiment (which is
not necessarily same as the one who registered the tool) can invite
judges to validate the results (Figure \ref{fig:registration_screens},
bottom). These judges must be registered users; \IC\ enforces this by
design.

Finally, Figure \ref{fig:evaluate_pairs_screen}, shows what is
perhaps the most important element of \IC: the manual validation of
clone pairs. This page is composed by a split screen with two
columns, showing both elements of a certain clone pair candidate. The
judge must then decide if this pair does indeed represent a clone or
not (if it is a true or a false positive). There are two optional form
elements: one to select the clone type, and another to leave a
comment. This is for situations in which user is sure that a pair is
indeed a clone, but has difficulty understanding its type. Note that
there is no option to label a clone pair as a Type I clone, since
these types are automatically detected through the mechanism described
in Section \ref{subsect:auto-type-2}.

\subsection{Thresholds for Classification}

The minimum accepted method size to consider a pair by \IC\ is that
both have 50 tokens as this is the minimum accepted size for clone
precision studies
~\cite{sajnani2016sourcerercc,Svajlenko:2015:ECD:2881297.2881379}. These
tokens are Java language tokens as defined in BCB. Within the context
of BCB, we only consider the clones that are detected with a syntactic
similarity of 70\% or more, the other ones we consider uncertain and
require the users to manually validate them, effectively treating them
as unknown.

One important consideration is the final labeling of a clone pair
candidate as a true or a false positive. Different experiments result
in different clone pairs being manually inspected. They also may result
in inspecting clone pairs that were already inspected in other
experiments, by other judges. \IC\ stores all judgements. However, it
has a high bar for accepting a label as final: the label on a given
clone pair is only considered final after 10 different unique votes,
and only if at least 70\% of them agree on the label. For any clone
pair candidate below this threshold, \IC\ will always require a manual
judgment. Note that this does not affect each individual
experimentation: a certain user can always be sure of the results
provided by \IC\ as long as he/she trusts his/her judges. This
consideration affects the internal information of \IC\ and is the
mechanism through which a certain pair is known (as, or as not, a
clone) and added to the body of knowledge.




==> problemstatement.tex <==
\section{Problem Statement}
\label{sect:probstate}

Recall and Precision metrics are two important metrics which are used to evaluate the detection performance of source code clone detectors. While there has been good progress with respect to measuring recall
systematically. Based on the BigCloneBench
dataset~\cite{Svajlenko:2014:TBD:2705615.2706134},
BigCloneEval~\cite{7816515} estimates recall automatically by
measuring how many of the labeled clone pairs are included in the
output of a clone detector. However, BigCloneEval stops short of
measuring precision because BigCloneBench does not contain labels for
{\em all} possible clone pairs in it. If a clone detector identifies a
clone pair that is not marked as such, only manual inspection can tell
whether the pair is a false positive or a true positive. So, while clone detectors that work in
Java typically report recall using BigCloneEval, the determination of
their precision is still a manual process, leading to difficulties in
comparing with other tools. In observing the literature on clone
detectors, and based on our own experience with code clone detection
tools, it is clear that the absence of an established labeled dataset
for precision creates a number of problems:

%use each tool is evaluated on a set of inputs that were created in the context of the research project by the necessity of having  a means of validation. This brings problems:

% (pedro) I think the first point is too frugal and the commented points should be added
% Maybe first point can be rephrase to identify sampling bias on the dataset (teams choose datasets they have good knowledge of etc)
\begin{itemize}
	\item Precision estimation can suffer from sampling bias. While sampling clone pairs, one needs to make sure that the sampling is carried out correctly to ensure the sample represents the population it is taken from.
	\item Large manual effort is required to conduct precision studies. As each pair in the sample needs to be evaluated, often by multiple judges, the total manual effort required to complete a precision study is big. 
	% Tool validation is idiosyncratic, rather than generic. It is often created by a team to evaluate their tool. It is subject to the proficiency of the team, to the information they have available, and unconscious human-bias\footnote{For example, sampling bias.}.
	\item The efforts put into the manual inspection of clone pairs have
	not been reused between studies. Every time a team wants to estimate precision of
	their tool, they typically start from scratch.
	%\item Inter-tool comparison becomes quite hard and somehow conjectural rather than based on a shared knowledge. It is easy to understand the pitfalls of comparing two tools by the results provided on the respective, idiosyncratic evaluations rather than by running them on the exact same input. This has the implication that it is, of now, quite hard to have a proper notion of the performance of the published tools and techniques in comparison with each other.
\end{itemize}

In this study 


==> validation.tex <==
\section{Assessment}
\label{sect:validation}

As stated before, our own work was partly the motivation for
developing \IC. In this section, we describe our comparative studies
of precision of three clone detectors: NiCad, CloneWorks, and
SourcererCC. Prior to developing \IC, these studies were done in
ad-hoc manner, and without reusing any information among
them. \IC\ allows us to streamline the process. 

NiCad and CloneWorks were already described in the previous
section. SourcererCC~\cite{sajnani2016sourcerercc}, similar to
CloneWorks, uses a hybrid of token-based and index-based approach to
detect clone pairs. Clone detection is carried out by querying the
partial-index of code blocks created by global token frequency map and
comparing code blocks based on the number of shared tokens between
them. In order to reduce the number of candidate pairs before doing
the comparison, two heuristics are applied: \textit{sub-block overlap
  filtering} based on the similarity threshold to compare a subset of
tokens within each block, and \textit{token position filtering} to
calculate an upper bound and a lower bound of similarity between two
blocks.

In order to run these tools, we followed the configurations defined
in~\cite{Svajlenko:2015:ECD:2881297.2881379} and in each tool's paper,
and we also consulted the tools' authors to get the right
configurations. The configurations for each tool are shown in Table
~\ref{fig:condig-tools}.

\begin{table*}[]
	\centering
	\caption{Configuration Settings for running SourcererCC, Nicad and CloneWorks.}
	\label{fig:condig-tools}
	\begin{tabular}{|l|l|}
		\hline
		\multicolumn{1}{|c|}{Tool}  & Run Configurations \\ \hline \hline
		Nicad                                   &      Min lines= 6, Difference threshold= 30\%, Rename= blind, Abstract= literal      \\ \hline
		CloneWorks                              & Min tokens= 1, Similarity threshold= 70\%, Mode= Aggressive        \\ \hline
		SourcererCC                            & Min tokens= 1, Similarity threshold= 70\%           \\ \hline
		
	\end{tabular}
\end{table*}

Comparing \IC\ to our previous ad-hoc precision studies serves a few purposes:

\begin{itemize}

\item \textbf{Feasibility and usability.} A precision study for 3 different tools and multiple judges is a non-trivial use of \IC. It allowed an assessment of the interface and usability, treatment and polishing of the source code and, more importantly, a confirmation that the tool works as intended.

\item \textbf{Accuracy.} Comparing \IC\ with the ad-hoc, labour-intensive process allows us to compare the values of precision with a baseline. Because of statistical variance, the results of different experiments are not expected to be exactly the same. But they should be statistically identical.

\item \textbf{Automatic labeling, in practice.} \IC\ is built on a database of known clone pairs, which expedites the process of large scale manual analysis. Furthermore, it also has mechanisms to automatically resolve Type I clones, and is loaded with a large set of known Type II clone pairs. This study serves therefore to understand how these constituents of \IC\ influence tool analysis in practice.

\end{itemize}

\subsection{Estimating Precision Without Using \IC}

In order to compare \IC\ results with the results of a manual effort
of measuring precision, we first start by manually analyzing the three
clone detectors, outside of \IC, in terms of their precision. To do
so, for each tool, we randomly sampled 400 clone pairs (ensuring size
of each code block $>=$ 50 tokens), a statistically significant sample
with 95\% confidence level and 5\% confidence interval, from the clone
pairs detected by each tool. The validation of clones were done by two
authors of this paper. The judges were blind from the source of each
clone pair. They followed the strict definitions of Type I, Type II,
Type III and Type IV clones in order to make their decisions. Wherever
there was a conflict between their judgments, they discussed the
conflict, and reached consensus by invoking the definitions.

The results obtained by the outside tool analysis of precision can be seen in Table \ref{fig:prec-rec-tools}.

\begin{table}[]
\centering
\caption{Precision of SourcererCC, Nicad and CloneWorks, with and
  without \IC.}
\label{fig:prec-rec-tools}
\begin{tabular}{lrrr}
\hline
\multicolumn{1}{|l|}{}    & \multicolumn{1}{l|}{SourcererCC}    & \multicolumn{1}{l|}{CloneWorks}  & \multicolumn{1}{l|}{NiCad} \\ \hline \hline
\multicolumn{1}{|l|}{Without \IC} & \multicolumn{1}{r|}{97.8\%} & \multicolumn{1}{r|}{98.7\%} & \multicolumn{1}{r|}{99\%}       \\ \hline
\multicolumn{1}{|l|}{With \IC} & \multicolumn{1}{r|}{97.5\%} & \multicolumn{1}{r|}{95.8\%} & \multicolumn{1}{r|}{97.3\%}       \\ \hline
\end{tabular}
\end{table}

\subsection{Estimating Precision With \IC}

To estimate precision of these tools with \IC, we created three
experiments in \IC, one for each tool. We uploaded the clone pairs
detected by each tool to their respective experiments in \IC, and for
each experiment three judges were responsible to validate the
necessary pairs. The precision value estimated by using \IC\ can also be
seen in Table \ref{fig:prec-rec-tools}.

%% \begin{table}[]
%% \centering
%% \caption{Precision of SourcererCC, Nicad and CloneWorks using InspectorClone. Clone values are only for the pairs that required manual validation, as seen in Table \ref{tab:pairs}.}
%% \label{fig:tools-eval}
%% \begin{tabular}{|l|r|r|r|}
%% \hline
%% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{SourcererCC} & \multicolumn{1}{c|}{Nicad} & \multicolumn{1}{c|}{CloneWorks} \\ \hline \hline
%% True Positives         & 187                      & 113                        & 134                             \\ \hline
%% False Positives        & 10                       & 17                         & 11                              \\ \hline
%% Precision              & 95.5\%                   & 95.8\%                     & 97.3\%                          \\ \hline
%% \end{tabular}
%% \end{table}


%There are a few things to note. First, the tools had small numbers of false positives. The automatic mechanism of Type I resolution and the pre-existence of known clone pairs might have helped achieving these results: because no one judges these cases, there is no possibility of having false negatives in them; however, we did not test this hypothesis~\com{(is the ambiguity resolved now? I'm not sure if I was able to make it clear)}. What is sure is that the task was facilitated compared to traditional, more naive approaches of tool precision validation.

The precision values achieved are very similar to the precision values that were described in Table \ref{fig:prec-rec-tools}. The difference in the values never goes past 3\% and can therefore be attributed to existing statistical deviations (margins of error). Given the small variances involved, we can say \IC\ provided correct results.

\subsection{Impact of Known Information}

The main advantage of using \IC\ can be seen in the amount of manual
labour involved in each case. In both cases, for each tool, 400 clone
pair candidates were sampled. In the case of ad-hoc evalutation, all
of these 400 pairs were evaluated by the judges. However, using
\IC, the judges were spared more than half of the samples, because
their labels were either already known, or were known during the
experiment. The amount of samples evaluated by judges can be seen in
Table \ref{tab:pairs}.

\begin{table}[]
	\centering
	\caption{Effort to estimate precision, in number of clone pair
          candidates shown to judges.}
	\label{tab:pairs}
	\begin{tabular}{|l|r|r|r|}
		\hline
		& \multicolumn{1}{l|}{SourcererCC} & \multicolumn{1}{l|}{CloneWorks} & \multicolumn{1}{l|}{NiCad} \\ \hline 
		Number of samples                  & 400                & 400                    & 400   \\ \hline \hline
		Without \IC  & 400                         & 400                    & 400               \\ \hline
		With \IC  & \textbf{197}             & \textbf{130}                    & \textbf{111}               \\ \hline
		%% Evaluated by BCB   & 6                      & 19                              & 155                        \\ \hline
		%% Evaluated by \IC\    & 197 (10)                      & 251 (6)                             & 134 (0)                        \\ \hline
	\end{tabular}
\end{table}

With \IC, the number of pairs requiring manual inspection ranged from
around 50\% of the total for SourcererCC to around 28\% of the total
for NiCad, which is a significant reduction in the amount of manual
effort. One might speculate that the results of CloneWorks and
NiCad are biased by the fact that these tools were used to populate the Type II clones pairs in the dataset (Section \ref{subsect:type2-addition}), but a close
observation proves otherwise: as it is visible in Table \ref{tab:autoval},
the vast majority of pairs automatically labeled by \IC\ were Type I.

\begin{table}[]
	\centering
	\caption{Number of pairs automatically validated in \IC,
          either by using BCB's database or by using the additional
          automatic classifiers in \IC. The numbers in parenthesis
          are Type II: for example, for SourcererCC,
          \IC\ automatically evaluated 197 candidate pairs, of which
          10 were Type II and the rest is Type I.}
	\label{tab:autoval}
	\begin{tabular}{|l|r|r|r|}
		\hline
		& \multicolumn{1}{l|}{SourcererCC} & \multicolumn{1}{l|}{CloneWorks} & \multicolumn{1}{l|}{NiCad} \\ \hline \hline
		Number of samples                  & 400                         & 400                    & 400               \\ \hline
		Labeled by BCB   & 6                      & 19                              & 155                        \\ \hline
		Labeled by \IC\    & 197 (10)                      & 251 (6)                             & 134 (0)                        \\ \hline
	\end{tabular}
\end{table}

These results show that \IC\ has a strong positive impact in
facilitating precision studies. We observed that in the worst case of
our experiments, with the use of \IC, 50\% of clone pairs needed human
validation effort, and the rest were automatically resolved by
\IC. The reduction
in manual effort will vary for each clone detector and also with
the progress in \IC's labeled dataset; over time we expect the manual effort to go further down.

%Hence, we can conclude that \IC\ can have a huge impact in the reduction of manual effort, probably depending on the tool being evaluated. Furthermore it is expected that the constant usage of tool over time will reduce these numbers further.

% (pedro) This section is maybe a little... hmm.. conceited (I think the word is cocky)
%% \subsection{Usability}

%% We did not perform a specific usability test, but it is worth leaving a note on the feedback of using \IC. The steps required to do the evaluation (registration, indication of judges, evaluation, and so on) were successfully used. The team had a few indications for improvement of the interface, some of them were corrected immediately (small bugs, typos, inter-browser compatibility issues, some polishing) and others are suggestions for future improvements (see Section \ref{sect:future}).

%% The general agreement, however, is that this method of semi-automated validation is much more preferable than more simplistic manual approaches. As our team itself has used those simple and manual approaches in the past, it was revealed that the advantages that \IC\ brings, go both towards the speed and ease of validation, and better and less error-prone results. Every member would prefer using \IC\ to any option experienced in the past.

